Gravitational realization of magnons in a ferromagnetic spin chain

A gravitational model of magnons in thermal equilibrium with a ferromagnetic spin chain is developed in a phenomenological bottom-up approach. A large Schwarzschild-AdS black hole background is used as the thermal reservoir and the magnon dynamics is obtained by scalar fields and branes in the bulk. The key feature of this model is that the coupling of the spin chain is related with the radial position in which the brane is located. We further study a ferromagnetic spin chain with a competing interaction and find that the couplings are related by the difference of positions of the branes. We show how to obtain the model from a weak limit of a dynamical gravitational system. This allows us to embed the model into a holographic system. The couplings can be related to entanglement entropy at finite temperature of the CFT since the turning point of minimal surfaces coincides with the position of the branes. The difference of entropy is used to define a notion of distance between the chain couplings.

==> FMSAdSref.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Rodrigo de Leon Ardon at 2019-12-13 13:31:45 -0600 


%% Saved with string encoding Unicode (UTF-8) 



@article{Swingle:2011np,
	Archiveprefix = {arXiv},
	Author = {Swingle, Brian and Senthil, T.},
	Date-Added = {2019-12-13 13:31:37 -0600},
	Date-Modified = {2019-12-13 13:31:37 -0600},
	Doi = {10.1103/PhysRevB.87.045123},
	Eprint = {1112.1069},
	Journal = {Phys. Rev.},
	Number = {4},
	Pages = {045123},
	Primaryclass = {cond-mat.str-el},
	Slaccitation = {%%CITATION = ARXIV:1112.1069;%%},
	Title = {{Universal crossovers between entanglement entropy and thermal entropy}},
	Volume = {B87},
	Year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevB.87.045123}}

@article{doi:10.1063/1.1664978,
	Author = {Majumdar,Chanchal K. and Ghosh,Dipan K.},
	Date-Added = {2019-12-13 09:50:06 -0600},
	Date-Modified = {2019-12-13 09:50:34 -0600},
	Doi = {10.1063/1.1664978},
	Journal = {Journal of Mathematical Physics},
	Number = {8},
	Pages = {1388-1398},
	Title = {On Next-Nearest-Neighbor Interaction in Linear Chain. I},
	Volume = {10},
	Year = {1969},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.1664978}}

@article{Beisert:2003tq,
	Archiveprefix = {arXiv},
	Author = {Beisert, N. and Kristjansen, C. and Staudacher, M.},
	Date-Added = {2019-12-13 09:12:31 -0600},
	Date-Modified = {2019-12-13 09:12:31 -0600},
	Doi = {10.1016/S0550-3213(03)00406-1},
	Eprint = {hep-th/0303060},
	Journal = {Nucl. Phys.},
	Pages = {131-184},
	Primaryclass = {hep-th},
	Reportnumber = {AEI-2003-028},
	Slaccitation = {%%CITATION = HEP-TH/0303060;%%},
	Title = {{The Dilatation operator of conformal N=4 superYang-Mills theory}},
	Volume = {B664},
	Year = {2003},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0550-3213(03)00406-1}}

@article{Kruczenski:2004kw,
	Archiveprefix = {arXiv},
	Author = {Kruczenski, M. and Ryzhov, A. V. and Tseytlin, Arkady A.},
	Date-Added = {2019-12-13 09:06:11 -0600},
	Date-Modified = {2019-12-13 09:06:53 -0600},
	Doi = {10.1016/j.nuclphysb.2004.05.028},
	Eprint = {hep-th/0403120},
	Journal = {Nucl. Phys.},
	Pages = {3-49},
	Primaryclass = {hep-th},
	Reportnumber = {BRX-TH-537},
	Slaccitation = {%%CITATION = HEP-TH/0403120;%%},
	Title = {{Large spin limit of $AdS_5 \times S^5$ string theory and low-energy expansion of ferromagnetic spin chains}},
	Volume = {B692},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.nuclphysb.2004.05.028}}

@article{Kruczenski:2003gt,
	Archiveprefix = {arXiv},
	Author = {Kruczenski, Martin},
	Date-Added = {2019-12-13 09:01:07 -0600},
	Date-Modified = {2019-12-13 09:01:07 -0600},
	Doi = {10.1103/PhysRevLett.93.161602},
	Eprint = {hep-th/0311203},
	Journal = {Phys. Rev. Lett.},
	Pages = {161602},
	Primaryclass = {hep-th},
	Reportnumber = {BRX-TH-539},
	Slaccitation = {%%CITATION = HEP-TH/0311203;%%},
	Title = {{Spin chains and string theory}},
	Volume = {93},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevLett.93.161602}}

@book{sachdev_2011,
	Author = {Sachdev, Subir},
	Date-Added = {2019-12-13 07:52:07 -0600},
	Date-Modified = {2019-12-13 07:52:07 -0600},
	Doi = {10.1017/CBO9780511973765},
	Edition = {2},
	Place = {Cambridge},
	Publisher = {Cambridge University Press},
	Title = {Quantum Phase Transitions},
	Year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1017/CBO9780511973765}}

@book{doi:10.1142/8676,
	Author = {Diep, H T},
	Date-Added = {2019-12-10 08:56:40 -0600},
	Date-Modified = {2019-12-10 09:52:17 -0600},
	Doi = {10.1142/8676},
	Edition = {2nd},
	Publisher = {WORLD SCIENTIFIC},
	Title = {Frustrated Spin Systems},
	Year = {2013},
	Bdsk-Url-1 = {https://www.worldscientific.com/doi/abs/10.1142/8676},
	Bdsk-Url-2 = {https://doi.org/10.1142/8676}}

@article{Calabrese:2009qy,
	Archiveprefix = {arXiv},
	Author = {Calabrese, Pasquale and Cardy, John},
	Date-Added = {2019-12-09 07:06:10 -0600},
	Date-Modified = {2019-12-09 07:06:10 -0600},
	Doi = {10.1088/1751-8113/42/50/504005},
	Eprint = {0905.4013},
	Journal = {J. Phys.},
	Pages = {504005},
	Primaryclass = {cond-mat.stat-mech},
	Slaccitation = {%%CITATION = ARXIV:0905.4013;%%},
	Title = {{Entanglement entropy and conformal field theory}},
	Volume = {A42},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1088/1751-8113/42/50/504005}}

@article{Hubeny:2012ry,
	Archiveprefix = {arXiv},
	Author = {Hubeny, Veronika E.},
	Date-Added = {2019-12-08 17:41:36 -0600},
	Date-Modified = {2019-12-08 17:41:36 -0600},
	Doi = {10.1007/JHEP07(2012)093},
	Eprint = {1203.1044},
	Journal = {JHEP},
	Pages = {093},
	Primaryclass = {hep-th},
	Reportnumber = {DCTP-12-15},
	Slaccitation = {%%CITATION = ARXIV:1203.1044;%%},
	Title = {{Extremal surfaces as bulk probes in AdS/CFT}},
	Volume = {07},
	Year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP07(2012)093}}

@inproceedings{Klebanov:2000me,
	Archiveprefix = {arXiv},
	Author = {Klebanov, Igor R.},
	Booktitle = {{Strings, branes and gravity. Proceedings, Theoretical Advanced Study Institute, TASI'99, Boulder, USA, May 31-June 25, 1999}},
	Date-Added = {2019-12-08 11:37:36 -0600},
	Date-Modified = {2019-12-08 11:37:36 -0600},
	Doi = {10.1142/9789812799630_0007},
	Eprint = {hep-th/0009139},
	Pages = {615-650},
	Primaryclass = {hep-th},
	Reportnumber = {PUPT-1954},
	Slaccitation = {%%CITATION = HEP-TH/0009139;%%},
	Title = {{TASI lectures: Introduction to the AdS / CFT correspondence}},
	Year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1142/9789812799630_0007}}

@article{Aharony:1999ti,
	Archiveprefix = {arXiv},
	Author = {Aharony, Ofer and Gubser, Steven S. and Maldacena, Juan Martin and Ooguri, Hirosi and Oz, Yaron},
	Date-Added = {2019-12-08 11:35:38 -0600},
	Date-Modified = {2019-12-08 11:35:38 -0600},
	Doi = {10.1016/S0370-1573(99)00083-6},
	Eprint = {hep-th/9905111},
	Journal = {Phys. Rept.},
	Pages = {183-386},
	Primaryclass = {hep-th},
	Reportnumber = {CERN-TH-99-122, HUTP-99-A027, LBNL-43113, RU-99-18, UCB-PTH-99-16, LBL-43113},
	Slaccitation = {%%CITATION = HEP-TH/9905111;%%},
	Title = {{Large N field theories, string theory and gravity}},
	Volume = {323},
	Year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0370-1573(99)00083-6}}

@inproceedings{DHoker:2002nbb,
	Archiveprefix = {arXiv},
	Author = {D'Hoker, Eric and Freedman, Daniel Z.},
	Booktitle = {{Strings, Branes and Extra Dimensions: TASI 2001: Proceedings}},
	Date-Added = {2019-12-08 11:33:29 -0600},
	Date-Modified = {2019-12-08 11:33:29 -0600},
	Eprint = {hep-th/0201253},
	Pages = {3-158},
	Primaryclass = {hep-th},
	Reportnumber = {UCLA-02-TEP-3, MIT-CTP-3242},
	Slaccitation = {%%CITATION = HEP-TH/0201253;%%},
	Title = {{Supersymmetric gauge theories and the AdS / CFT correspondence}},
	Year = {2002}}

@book{Nastase:2017cxp,
	Author = {Nastase, Horatiu},
	Date-Added = {2019-12-08 10:50:23 -0600},
	Date-Modified = {2019-12-08 10:50:23 -0600},
	Doi = {10.1017/9781316847978},
	Isbn = {9781316853047, 9781107180383},
	Publisher = {Cambridge University Press},
	Slaccitation = {%%CITATION = INSPIRE-1638019;%%},
	Title = {{String Theory Methods for Condensed Matter Physics}},
	Url = {http://www.cambridge.org/academic/subjects/physics/theoretical-physics-and-mathematical-physics/string-theory-methods-condensed-matter-physics?format=AR&isbn=9781316853047},
	Year = {2017},
	Bdsk-Url-1 = {http://www.cambridge.org/academic/subjects/physics/theoretical-physics-and-mathematical-physics/string-theory-methods-condensed-matter-physics?format=AR&isbn=9781316853047},
	Bdsk-Url-2 = {https://doi.org/10.1017/9781316847978}}

@article{Zarembo:2004hp,
	Archiveprefix = {arXiv},
	Author = {Zarembo, K.},
	Booktitle = {{International Workshop on Integrable Models and Applications: 2nd Annual Meeting of the EU Network EUCLID Sozopol, Bulgaria, August 31-September 4, 2004}},
	Date-Added = {2019-12-07 18:39:05 -0600},
	Date-Modified = {2019-12-07 18:39:05 -0600},
	Doi = {10.1002/prop.200410233},
	Eprint = {hep-th/0411191},
	Journal = {Comptes Rendus Physique},
	Note = {[Fortsch. Phys.53,647(2005)]},
	Pages = {1081-1090},
	Primaryclass = {hep-th},
	Reportnumber = {UUITP-27-04, ITEP-TH-50-04},
	Slaccitation = {%%CITATION = HEP-TH/0411191;%%},
	Title = {{Semiclassical Bethe Ansatz and AdS/CFT}},
	Volume = {5},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1002/prop.200410233}}

@article{Minahan:2002ve,
	Archiveprefix = {arXiv},
	Author = {Minahan, J. A. and Zarembo, K.},
	Date-Added = {2019-12-07 18:33:12 -0600},
	Date-Modified = {2019-12-07 18:33:12 -0600},
	Doi = {10.1088/1126-6708/2003/03/013},
	Eprint = {hep-th/0212208},
	Journal = {JHEP},
	Pages = {013},
	Primaryclass = {hep-th},
	Reportnumber = {UUITP-17-02, ITEP-TH-73-02},
	Slaccitation = {%%CITATION = HEP-TH/0212208;%%},
	Title = {{The Bethe ansatz for N=4 superYang-Mills}},
	Volume = {03},
	Year = {2003},
	Bdsk-Url-1 = {https://doi.org/10.1088/1126-6708/2003/03/013}}

@book{AshMermin,
	Author = {Neil W. Ashcroft and N. David Mermin},
	Date-Added = {2019-12-06 19:06:19 -0600},
	Date-Modified = {2019-12-06 19:08:30 -0600},
	Publisher = {Harcourt College},
	Title = {Solid State Physics},
	Year = {1976}}

@article{Hofman:2006xt,
	Archiveprefix = {arXiv},
	Author = {Hofman, Diego M. and Maldacena, Juan Martin},
	Date-Added = {2019-12-05 23:32:25 -0600},
	Date-Modified = {2019-12-05 23:32:25 -0600},
	Doi = {10.1088/0305-4470/39/41/S17},
	Eprint = {hep-th/0604135},
	Journal = {J. Phys.},
	Pages = {13095-13118},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = HEP-TH/0604135;%%},
	Title = {{Giant Magnons}},
	Volume = {A39},
	Year = {2006},
	Bdsk-Url-1 = {https://doi.org/10.1088/0305-4470/39/41/S17}}

@article{Filev:2009xp,
	Archiveprefix = {arXiv},
	Author = {Filev, Veselin G. and Johnson, Clifford V. and Shock, Jonathan P.},
	Date-Added = {2019-12-05 23:24:43 -0600},
	Date-Modified = {2019-12-05 23:24:43 -0600},
	Doi = {10.1088/1126-6708/2009/08/013},
	Eprint = {0903.5345},
	Journal = {JHEP},
	Pages = {013},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:0903.5345;%%},
	Title = {{Universal Holographic Chiral Dynamics in an External Magnetic Field}},
	Volume = {08},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1088/1126-6708/2009/08/013}}

@article{Rangamani:2016dms,
	Archiveprefix = {arXiv},
	Author = {Rangamani, Mukund and Takayanagi, Tadashi},
	Date-Added = {2019-12-05 13:48:04 -0600},
	Date-Modified = {2019-12-05 13:48:04 -0600},
	Doi = {10.1007/978-3-319-52573-0},
	Eprint = {1609.01287},
	Journal = {Lect. Notes Phys.},
	Pages = {pp.1-246},
	Primaryclass = {hep-th},
	Reportnumber = {YITP-16-106},
	Slaccitation = {%%CITATION = ARXIV:1609.01287;%%},
	Title = {{Holographic Entanglement Entropy}},
	Volume = {931},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-3-319-52573-0}}

@article{Elvang:2016tzz,
	Archiveprefix = {arXiv},
	Author = {Elvang, Henriette and Hadjiantonis, Marios},
	Date-Added = {2019-12-03 21:25:04 -0600},
	Date-Modified = {2019-12-03 21:25:04 -0600},
	Doi = {10.1007/JHEP06(2016)046},
	Eprint = {1603.04485},
	Journal = {JHEP},
	Pages = {046},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1603.04485;%%},
	Title = {{A Practical Approach to the Hamilton-Jacobi Formulation of Holographic Renormalization}},
	Volume = {06},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP06(2016)046}}

@article{Balasubramanian:1999re,
	Archiveprefix = {arXiv},
	Author = {Balasubramanian, Vijay and Kraus, Per},
	Date-Added = {2019-12-03 21:17:52 -0600},
	Date-Modified = {2019-12-03 21:17:52 -0600},
	Doi = {10.1007/s002200050764},
	Eprint = {hep-th/9902121},
	Journal = {Commun. Math. Phys.},
	Pages = {413-428},
	Primaryclass = {hep-th},
	Reportnumber = {HUTP-99-A002, EFI-99-6, NSF-ITP-98-132},
	Slaccitation = {%%CITATION = HEP-TH/9902121;%%},
	Title = {{A Stress tensor for Anti-de Sitter gravity}},
	Volume = {208},
	Year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.1007/s002200050764}}

@article{Weinberg:1993dw,
	Archiveprefix = {arXiv},
	Author = {Weinberg, Steven},
	Date-Added = {2019-12-02 15:34:33 -0600},
	Date-Modified = {2019-12-02 15:34:33 -0600},
	Doi = {10.1016/0550-3213(94)90001-9},
	Eprint = {cond-mat/9306055},
	Journal = {Nucl. Phys.},
	Pages = {567-578},
	Primaryclass = {cond-mat},
	Reportnumber = {UTTG-18-93},
	Slaccitation = {%%CITATION = COND-MAT/9306055;%%},
	Title = {{Effective action and renormalization group flow of anisotropic superconductors}},
	Volume = {B413},
	Year = {1994},
	Bdsk-Url-1 = {https://doi.org/10.1016/0550-3213(94)90001-9}}

@article{Natsuume:2014sfa,
	Archiveprefix = {arXiv},
	Author = {Natsuume, Makoto},
	Date-Added = {2019-11-29 18:16:34 -0600},
	Date-Modified = {2019-11-29 18:16:34 -0600},
	Doi = {10.1007/978-4-431-55441-7},
	Eprint = {1409.3575},
	Journal = {Lect. Notes Phys.},
	Pages = {pp.1-294},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1409.3575;%%},
	Title = {{AdS/CFT Duality User Guide}},
	Volume = {903},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1007/978-4-431-55441-7}}

@article{1973CMaPh..31..259C,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/1973CMaPh..31..259C},
	Author = {{Coleman}, Sidney},
	Date-Added = {2019-11-29 13:44:06 -0600},
	Date-Modified = {2019-11-29 13:44:06 -0600},
	Doi = {10.1007/BF01646487},
	Journal = {Communications in Mathematical Physics},
	Month = {Dec},
	Number = {4},
	Pages = {259-264},
	Title = {{There are no Goldstone bosons in two dimensions}},
	Volume = {31},
	Year = {1973},
	Bdsk-Url-1 = {https://doi.org/10.1007/BF01646487}}

@article{PhysRevLett.17.1133,
	Author = {Mermin, N. D. and Wagner, H.},
	Date-Added = {2019-11-29 13:43:20 -0600},
	Date-Modified = {2019-11-29 13:43:20 -0600},
	Doi = {10.1103/PhysRevLett.17.1133},
	Issue = {22},
	Journal = {Phys. Rev. Lett.},
	Month = {Nov},
	Numpages = {0},
	Pages = {1133--1136},
	Publisher = {American Physical Society},
	Title = {Absence of Ferromagnetism or Antiferromagnetism in One- or Two-Dimensional Isotropic Heisenberg Models},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.17.1133},
	Volume = {17},
	Year = {1966},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.17.1133},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.17.1133}}

@article{DW75,
	Author = {Dembinski, S. T. and Wydro, T.},
	Date-Added = {2019-11-29 12:10:50 -0600},
	Date-Modified = {2019-11-29 12:11:22 -0600},
	Doi = {10.1002/pssb.2220670246},
	Eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/pssb.2220670246},
	Journal = {physica status solidi (b)},
	Number = {2},
	Pages = {K123-K126},
	Title = {Linear quantum-classical heisenberg model},
	Url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/pssb.2220670246},
	Volume = {67},
	Year = {1975},
	Bdsk-Url-1 = {https://onlinelibrary.wiley.com/doi/abs/10.1002/pssb.2220670246},
	Bdsk-Url-2 = {https://doi.org/10.1002/pssb.2220670246}}

@article{BloteH79,
	Author = {Bl\"ote,H. W. J.},
	Date-Added = {2019-11-29 11:58:44 -0600},
	Date-Modified = {2019-11-29 12:00:09 -0600},
	Doi = {10.1063/1.326907},
	Eprint = {https://aip.scitation.org/doi/pdf/10.1063/1.326907},
	Journal = {Journal of Applied Physics},
	Number = {B11},
	Pages = {7401-7403},
	Title = {Heisenberg chains with alternating spin quantum numbers},
	Url = {https://aip.scitation.org/doi/abs/10.1063/1.326907},
	Volume = {50},
	Year = {1979},
	Bdsk-Url-1 = {https://aip.scitation.org/doi/abs/10.1063/1.326907},
	Bdsk-Url-2 = {https://doi.org/10.1063/1.326907}}

@book{AAFerro,
	Author = {Aharoni, Amikan},
	Date-Added = {2019-11-29 11:30:39 -0600},
	Date-Modified = {2019-11-29 11:33:00 -0600},
	Edition = {2},
	Isbn = {978-0198508090},
	Publisher = {Oxford University Press},
	Series = {International Series of Monographs on Physics},
	Title = {An Introduction to the Theory of Ferromagnetism},
	Year = {2000}}

@article{HU2015539,
	Author = {Ai-Yuan Hu and Zhi-Min Wu and Yu-Ting Cui and Guo-Ping Qin},
	Date-Added = {2019-11-29 11:18:25 -0600},
	Date-Modified = {2019-11-29 11:18:41 -0600},
	Doi = {https://doi.org/10.1016/j.jmmm.2014.09.010},
	Issn = {0304-8853},
	Journal = {Journal of Magnetism and Magnetic Materials},
	Pages = {539 - 543},
	Title = {The paramagnetic properties of ferromagnetic mixed-spin chain system},
	Url = {http://www.sciencedirect.com/science/article/pii/S0304885314008294},
	Volume = {374},
	Year = {2015},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0304885314008294},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.jmmm.2014.09.010}}

@article{Fukushima_2004,
	Author = {Fukushima, Noboru and Honecker, Andreas and Wessel, Stefan and Brenig, Wolfram},
	Date-Added = {2019-11-29 11:10:15 -0600},
	Date-Modified = {2019-11-29 11:10:15 -0600},
	Doi = {10.1103/physrevb.69.174430},
	Issn = {1550-235X},
	Journal = {Physical Review B},
	Month = {May},
	Number = {17},
	Publisher = {American Physical Society (APS)},
	Title = {Thermodynamic properties of ferromagnetic mixed-spin chain systems},
	Url = {http://dx.doi.org/10.1103/PhysRevB.69.174430},
	Volume = {69},
	Year = {2004},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevB.69.174430},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevb.69.174430}}

@article{Agrapidis_2019,
	Author = {Agrapidis, Cli{\`o} Efthimia and Drechsler, Stefan-Ludwig and van den Brink, Jeroen and Nishimoto, Satoshi},
	Date-Added = {2019-11-29 10:51:43 -0600},
	Date-Modified = {2019-11-29 10:51:43 -0600},
	Doi = {10.21468/scipostphys.6.2.019},
	Journal = {SciPost Physics},
	Month = {Feb},
	Number = {2},
	Publisher = {Stichting SciPost},
	Title = {Coexistence of valence-bond formation and topological order in the Frustrated Ferromagnetic $J_1$-$J_2$ Chain},
	Url = {http://dx.doi.org/10.21468/SciPostPhys.6.2.019},
	Volume = {6},
	Year = {2019},
	Bdsk-Url-1 = {http://dx.doi.org/10.21468/SciPostPhys.6.2.019},
	Bdsk-Url-2 = {http://dx.doi.org/10.21468/scipostphys.6.2.019}}

@article{Kecke_2007,
	Author = {Kecke, Lars and Momoi, Tsutomu and Furusaki, Akira},
	Date-Added = {2019-11-29 10:50:31 -0600},
	Date-Modified = {2019-11-29 10:50:31 -0600},
	Doi = {10.1103/physrevb.76.060407},
	Issn = {1550-235X},
	Journal = {Physical Review B},
	Month = {Aug},
	Number = {6},
	Publisher = {American Physical Society (APS)},
	Title = {Multimagnon bound states in the frustrated ferromagnetic one-dimensional chain},
	Url = {http://dx.doi.org/10.1103/PhysRevB.76.060407},
	Volume = {76},
	Year = {2007},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevB.76.060407},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevb.76.060407}}

@article{Gubser:1998bc,
	Archiveprefix = {arXiv},
	Author = {Gubser, S. S. and Klebanov, Igor R. and Polyakov, Alexander M.},
	Date-Added = {2019-11-29 08:53:28 -0600},
	Date-Modified = {2019-11-29 08:53:28 -0600},
	Doi = {10.1016/S0370-2693(98)00377-3},
	Eprint = {hep-th/9802109},
	Journal = {Phys. Lett.},
	Pages = {105-114},
	Primaryclass = {hep-th},
	Reportnumber = {PUPT-1767},
	Slaccitation = {%%CITATION = HEP-TH/9802109;%%},
	Title = {{Gauge theory correlators from noncritical string theory}},
	Volume = {B428},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0370-2693(98)00377-3}}

@article{Cai:2014oca,
	Archiveprefix = {arXiv},
	Author = {Cai, Rong-Gen and Yang, Run-Qiu},
	Date-Added = {2019-11-29 08:43:46 -0600},
	Date-Modified = {2019-11-29 08:43:46 -0600},
	Doi = {10.1103/PhysRevD.90.081901},
	Eprint = {1404.2856},
	Journal = {Phys. Rev.},
	Number = {8},
	Pages = {081901},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1404.2856;%%},
	Title = {{Paramagnetism-Ferromagnetism Phase Transition in a Dyonic Black Hole}},
	Volume = {D90},
	Year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.90.081901}}

@article{Cai:2015jta,
	Archiveprefix = {arXiv},
	Author = {Cai, Rong-Gen and Yang, Run-Qiu and Wu, Ya-Bo and Zhang, Cheng-Yuan},
	Date-Added = {2019-11-29 08:43:23 -0600},
	Date-Modified = {2019-11-29 08:43:23 -0600},
	Doi = {10.1007/JHEP11(2015)021},
	Eprint = {1507.00546},
	Journal = {JHEP},
	Pages = {021},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1507.00546;%%},
	Title = {{Massive $2$-form field and holographic ferromagnetic phase transition}},
	Volume = {11},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP11(2015)021}}

@article{Iqbal:2010eh,
	Archiveprefix = {arXiv},
	Author = {Iqbal, Nabil and Liu, Hong and Mezei, Mark and Si, Qimiao},
	Date-Added = {2019-11-29 08:39:47 -0600},
	Date-Modified = {2019-11-29 08:39:47 -0600},
	Doi = {10.1103/PhysRevD.82.045002},
	Eprint = {1003.0010},
	Journal = {Phys. Rev.},
	Pages = {045002},
	Primaryclass = {hep-th},
	Reportnumber = {MIT-CTP-4126},
	Slaccitation = {%%CITATION = ARXIV:1003.0010;%%},
	Title = {{Quantum phase transitions in holographic models of magnetism and superconductors}},
	Volume = {D82},
	Year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.82.045002}}

@article{Yokoi:2015qba,
	Archiveprefix = {arXiv},
	Author = {Yokoi, Naoto and Ishihara, Masafumi and Sato, Koji and Saitoh, Eiji},
	Date-Added = {2019-11-29 08:33:28 -0600},
	Date-Modified = {2019-11-29 08:33:28 -0600},
	Doi = {10.1103/PhysRevD.93.026002},
	Eprint = {1508.01626},
	Journal = {Phys. Rev.},
	Number = {2},
	Pages = {026002},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1508.01626;%%},
	Title = {{Holographic realization of ferromagnets}},
	Volume = {D93},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.93.026002}}

@book{kittelbook,
	Author = {Charles Kittel},
	Date-Added = {2019-11-28 21:53:30 -0600},
	Date-Modified = {2019-11-28 21:55:50 -0600},
	Edition = {8},
	Number = {978-0-471-41526-8},
	Publisher = {Wiley},
	Title = {Introduction to Solid State Physics},
	Year = {2004}}

@article{Hartnoll:2016apf,
	Archiveprefix = {arXiv},
	Author = {Hartnoll, Sean A. and Lucas, Andrew and Sachdev, Subir},
	Date-Added = {2019-11-28 21:20:09 -0600},
	Date-Modified = {2019-11-28 21:20:09 -0600},
	Eprint = {1612.07324},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1612.07324;%%},
	Title = {{Holographic quantum matter}},
	Year = {2016}}

@article{Witten:1998qj,
	Archiveprefix = {arXiv},
	Author = {Witten, Edward},
	Date-Added = {2019-11-28 20:53:20 -0600},
	Date-Modified = {2019-11-28 20:53:20 -0600},
	Doi = {10.4310/ATMP.1998.v2.n2.a2},
	Eprint = {hep-th/9802150},
	Journal = {Adv. Theor. Math. Phys.},
	Pages = {253-291},
	Primaryclass = {hep-th},
	Reportnumber = {IASSNS-HEP-98-15},
	Slaccitation = {%%CITATION = HEP-TH/9802150;%%},
	Title = {{Anti-de Sitter space and holography}},
	Volume = {2},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.4310/ATMP.1998.v2.n2.a2}}

@article{Maldacena:1997re,
	Archiveprefix = {arXiv},
	Author = {Maldacena, Juan Martin},
	Date-Added = {2019-11-28 20:52:06 -0600},
	Date-Modified = {2019-11-28 20:52:06 -0600},
	Doi = {10.1023/A:1026654312961, 10.4310/ATMP.1998.v2.n2.a1},
	Eprint = {hep-th/9711200},
	Journal = {Int. J. Theor. Phys.},
	Note = {[Adv. Theor. Math. Phys.2,231(1998)]},
	Pages = {1113-1133},
	Primaryclass = {hep-th},
	Reportnumber = {HUTP-97-A097, HUTP-98-A097},
	Slaccitation = {%%CITATION = HEP-TH/9711200;%%},
	Title = {{The Large N limit of superconformal field theories and supergravity}},
	Volume = {38},
	Year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.1023/A:1026654312961,%2010.4310/ATMP.1998.v2.n2.a1}}

@article{Hawking:1982dh,
	Author = {Hawking, S. W. and Page, Don N.},
	Date-Added = {2019-11-28 11:13:14 -0600},
	Date-Modified = {2019-11-28 11:13:14 -0600},
	Doi = {10.1007/BF01208266},
	Journal = {Commun. Math. Phys.},
	Pages = {577},
	Reportnumber = {PRINT-83-0019 (CAMBRIDGE)},
	Slaccitation = {%%CITATION = CMPHA,87,577;%%},
	Title = {{Thermodynamics of Black Holes in anti-De Sitter Space}},
	Volume = {87},
	Year = {1983},
	Bdsk-Url-1 = {https://doi.org/10.1007/BF01208266}}

@article{Kubiznak:2016qmn,
	Archiveprefix = {arXiv},
	Author = {Kubiznak, David and Mann, Robert B. and Teo, Mae},
	Date-Added = {2019-11-28 10:35:08 -0600},
	Date-Modified = {2019-11-28 10:35:08 -0600},
	Doi = {10.1088/1361-6382/aa5c69},
	Eprint = {1608.06147},
	Journal = {Class. Quant. Grav.},
	Number = {6},
	Pages = {063001},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1608.06147;%%},
	Title = {{Black hole chemistry: thermodynamics with Lambda}},
	Volume = {34},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1088/1361-6382/aa5c69}}

@article{Hubeny:2009rc,
	Archiveprefix = {arXiv},
	Author = {Hubeny, Veronika E. and Marolf, Donald and Rangamani, Mukund},
	Date-Added = {2019-11-28 09:42:04 -0600},
	Date-Modified = {2019-11-28 09:42:04 -0600},
	Doi = {10.1088/0264-9381/27/9/095018},
	Eprint = {0911.4144},
	Journal = {Class. Quant. Grav.},
	Pages = {095018},
	Primaryclass = {hep-th},
	Reportnumber = {DCPT-09-77, NSF-KITP-09-204},
	Slaccitation = {%%CITATION = ARXIV:0911.4144;%%},
	Title = {{Hawking radiation from AdS black holes}},
	Volume = {27},
	Year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1088/0264-9381/27/9/095018}}

@article{Hemming:2007yq,
	Archiveprefix = {arXiv},
	Author = {Hemming, Samuli and Thorlacius, Larus},
	Date-Added = {2019-11-28 09:41:10 -0600},
	Date-Modified = {2019-11-28 09:41:10 -0600},
	Doi = {10.1088/1126-6708/2007/11/086},
	Eprint = {0709.3738},
	Journal = {JHEP},
	Pages = {086},
	Primaryclass = {hep-th},
	Reportnumber = {RH-05-2007},
	Slaccitation = {%%CITATION = ARXIV:0709.3738;%%},
	Title = {{Thermodynamics of Large AdS Black Holes}},
	Volume = {11},
	Year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1088/1126-6708/2007/11/086}}

@article{Brynjolfsson:2008uc,
	Archiveprefix = {arXiv},
	Author = {Brynjolfsson, Erling J. and Thorlacius, Larus},
	Date-Added = {2019-11-28 09:40:22 -0600},
	Date-Modified = {2019-11-28 09:40:22 -0600},
	Doi = {10.1088/1126-6708/2008/09/066},
	Eprint = {0805.1876},
	Journal = {JHEP},
	Pages = {066},
	Primaryclass = {hep-th},
	Reportnumber = {NORDITA-2008-16, RH-04-2008},
	Slaccitation = {%%CITATION = ARXIV:0805.1876;%%},
	Title = {{Taking the Temperature of a Black Hole}},
	Volume = {09},
	Year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1088/1126-6708/2008/09/066}}

@article{Jeske_2018,
	Author = {Jeske, Jan and Rivas, {\'A}ngel and Ahmed, Muhammad H and Martin-Delgado, Miguel A and Cole, Jared H},
	Date-Added = {2019-11-21 15:08:20 -0600},
	Date-Modified = {2019-11-21 15:08:20 -0600},
	Doi = {10.1088/1367-2630/aadecf},
	Issn = {1367-2630},
	Journal = {New Journal of Physics},
	Month = {Sep},
	Number = {9},
	Pages = {093017},
	Publisher = {IOP Publishing},
	Title = {The effects of thermal and correlated noise on magnons in a quantum ferromagnet},
	Url = {http://dx.doi.org/10.1088/1367-2630/aadecf},
	Volume = {20},
	Year = {2018},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/1367-2630/aadecf}}

@article{PhysRevB.46.8206,
	Author = {Ivanov, N. B. and Ivanov, P. Ch.},
	Date-Added = {2019-11-18 08:23:37 -0600},
	Date-Modified = {2019-11-18 08:23:37 -0600},
	Doi = {10.1103/PhysRevB.46.8206},
	Issue = {13},
	Journal = {Phys. Rev. B},
	Month = {Oct},
	Numpages = {0},
	Pages = {8206--8213},
	Publisher = {American Physical Society},
	Title = {Frustrated two-dimensional quantum Heisenberg antiferromagnet at low temperatures},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.46.8206},
	Volume = {46},
	Year = {1992},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.46.8206},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.46.8206}}

@article{PhysRevB.39.2344,
	Author = {Chakravarty, Sudip and Halperin, Bertrand I. and Nelson, David R.},
	Date-Added = {2019-11-18 08:22:02 -0600},
	Date-Modified = {2019-11-18 08:22:02 -0600},
	Doi = {10.1103/PhysRevB.39.2344},
	Issue = {4},
	Journal = {Phys. Rev. B},
	Month = {Feb},
	Numpages = {0},
	Pages = {2344--2371},
	Publisher = {American Physical Society},
	Title = {Two-dimensional quantum Heisenberg antiferromagnet at low temperatures},
	Url = {https://link.aps.org/doi/10.1103/PhysRevB.39.2344},
	Volume = {39},
	Year = {1989},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevB.39.2344},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevB.39.2344}}

@article{HALDANE1983464,
	Author = {F.D.M. Haldane},
	Date-Added = {2019-11-18 08:11:00 -0600},
	Date-Modified = {2019-11-18 08:11:12 -0600},
	Doi = {https://doi.org/10.1016/0375-9601(83)90631-X},
	Issn = {0375-9601},
	Journal = {Physics Letters A},
	Number = {9},
	Pages = {464 - 468},
	Title = {Continuum dynamics of the 1-D Heisenberg antiferromagnet: Identification with the O(3) nonlinear sigma model},
	Url = {http://www.sciencedirect.com/science/article/pii/037596018390631X},
	Volume = {93},
	Year = {1983},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/037596018390631X},
	Bdsk-Url-2 = {https://doi.org/10.1016/0375-9601(83)90631-X}}

@article{PhysRevLett.74.813,
	Author = {Dandoloff, R. and Villain-Guillot, S. and Saxena, A. and Bishop, A. R.},
	Date-Added = {2019-11-15 15:14:02 -0600},
	Date-Modified = {2019-11-15 15:14:02 -0600},
	Doi = {10.1103/PhysRevLett.74.813},
	Issue = {5},
	Journal = {Phys. Rev. Lett.},
	Month = {Jan},
	Numpages = {0},
	Pages = {813--815},
	Publisher = {American Physical Society},
	Title = {Violation of Self-Duality for Topological Solitons due to Soliton-Soliton Interaction on a Cylindrical Geometry},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.74.813},
	Volume = {74},
	Year = {1995},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.74.813},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.74.813}}

@article{CARVALHOSANTOS20131308,
	Author = {V.L. Carvalho-Santos and F.A. Apolonio and N.M. Oliveira-Neto},
	Date-Added = {2019-11-14 08:29:47 -0600},
	Date-Modified = {2019-11-14 08:29:58 -0600},
	Doi = {https://doi.org/10.1016/j.physleta.2013.03.028},
	Issn = {0375-9601},
	Journal = {Physics Letters A},
	Keywords = {Classical spin models, Solitons, Vortices, Curvature, Heisenberg model},
	Number = {18},
	Pages = {1308 - 1316},
	Title = {On geometry-dependent vortex stability and topological spin excitations on curved surfaces with cylindrical symmetry},
	Url = {http://www.sciencedirect.com/science/article/pii/S0375960113002995},
	Volume = {377},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0375960113002995},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.physleta.2013.03.028}}

@article{CARVALHOSANTOS20123551,
	Author = {Vagson L. Carvalho-Santos and Rossen Dandoloff},
	Date-Added = {2019-11-14 08:27:15 -0600},
	Date-Modified = {2019-11-14 08:27:26 -0600},
	Doi = {https://doi.org/10.1016/j.physleta.2012.10.027},
	Issn = {0375-9601},
	Journal = {Physics Letters A},
	Keywords = {Classical spin models, Skyrmions, Curvature, Heisenberg Hamiltonian},
	Number = {46},
	Pages = {3551 - 3554},
	Title = {Coupling between magnetic field and curvature in Heisenberg spins on surfaces with rotational symmetry},
	Url = {http://www.sciencedirect.com/science/article/pii/S0375960112010559},
	Volume = {376},
	Year = {2012},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0375960112010559},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.physleta.2012.10.027}}

@article{Dandoloff_2010,
	Abstract = {We obtain a half-skyrmion solution in the orientation of Heisenberg spins on a neck joining two planes with a semi-circular region. In addition, we consider several geometries, topologically equivalent to either a plane with a hole or a truncated circular cone or a cylinder due to the presence of an intrinsic length scale, for which we obtain skyrmion solutions. We also consider two minimal surfaces, namely a catenoid and a helicoid. Finally, we consider Heisenberg spins on single-sheet paraboloid and hyperboloid geometries. These spin textures may possibly be realized in elastically soft, curved magnetic thin films.},
	Author = {Rossen Dandoloff and Avadh Saxena},
	Date-Added = {2019-11-14 08:24:52 -0600},
	Date-Modified = {2019-11-14 08:24:52 -0600},
	Doi = {10.1088/1751-8113/44/4/045203},
	Journal = {Journal of Physics A: Mathematical and Theoretical},
	Month = {dec},
	Number = {4},
	Pages = {045203},
	Publisher = {{IOP} Publishing},
	Title = {Heisenberg spins on a bilayer connected by a neck and other geometries with a characteristic length scale},
	Url = {https://doi.org/10.1088%2F1751-8113%2F44%2F4%2F045203},
	Volume = {44},
	Year = 2010,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F1751-8113%2F44%2F4%2F045203},
	Bdsk-Url-2 = {https://doi.org/10.1088/1751-8113/44/4/045203}}

@article{DANDOLOFF2006421,
	Author = {Rossen Dandoloff and Avadh Saxena},
	Date-Added = {2019-11-14 08:18:09 -0600},
	Date-Modified = {2019-11-14 08:18:18 -0600},
	Doi = {https://doi.org/10.1016/j.physleta.2006.05.079},
	Issn = {0375-9601},
	Journal = {Physics Letters A},
	Number = {5},
	Pages = {421 - 425},
	Title = {XY-model on planar and space curves},
	Url = {http://www.sciencedirect.com/science/article/pii/S037596010600853X},
	Volume = {358},
	Year = {2006},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S037596010600853X},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.physleta.2006.05.079}}

@article{BENOIT1998439,
	Author = {J. Benoit and R. Dandoloff},
	Date-Added = {2019-11-14 08:10:53 -0600},
	Date-Modified = {2019-11-14 08:12:02 -0600},
	Doi = {https://doi.org/10.1016/S0375-9601(98)00657-4},
	Issn = {0375-9601},
	Journal = {Physics Letters A},
	Number = {5},
	Pages = {439 - 444},
	Title = {Heisenberg spins on an elastic torus section},
	Url = {http://www.sciencedirect.com/science/article/pii/S0375960198006574},
	Volume = {248},
	Year = {1998},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0375960198006574},
	Bdsk-Url-2 = {https://doi.org/10.1016/S0375-9601(98)00657-4}}

@proceedings{Affleck:1988mua,
	Author = {Affleck, I.},
	Date-Added = {2019-11-11 14:36:37 -0600},
	Date-Modified = {2019-11-11 14:36:37 -0600},
	Editor = {Brezin, E. and Zinn-Justin, J.},
	Organization = {North-Holland},
	Pages = {563},
	Publisher = {North-Holland},
	Series = {Les Houches 1988, Proceedings, Fields, strings and critical phenomena},
	Slaccitation = {%%CITATION = INSPIRE-1236260;%%},
	Title = {{Field Theory Methods and Quantum Critical Phenomena}},
	Year = {1988}}

@article{Bykov:2012am,
	Archiveprefix = {arXiv},
	Author = {Bykov, Dmitri},
	Date-Added = {2019-11-11 10:04:00 -0600},
	Date-Modified = {2019-11-11 10:04:00 -0600},
	Doi = {10.1007/s00220-013-1702-5},
	Eprint = {1206.2777},
	Journal = {Commun. Math. Phys.},
	Pages = {807-834},
	Primaryclass = {hep-th},
	Reportnumber = {NORDITA-2012-47},
	Slaccitation = {%%CITATION = ARXIV:1206.2777;%%},
	Title = {{The geometry of antiferromagnetic spin chains}},
	Volume = {322},
	Year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1007/s00220-013-1702-5}}

@misc{rao2005nonlinear,
	Archiveprefix = {arXiv},
	Author = {Sumathi Rao},
	Date-Added = {2019-11-11 10:00:50 -0600},
	Date-Modified = {2019-11-11 10:00:50 -0600},
	Eprint = {cond-mat/0512085},
	Primaryclass = {cond-mat.stat-mech},
	Title = {Non-linear sigma model approach to quantum spin chains},
	Year = {2005}}

@article{PhysRevLett.50.1153,
	Author = {Haldane, F. D. M.},
	Date-Added = {2019-11-10 08:39:08 -0600},
	Date-Modified = {2019-11-10 08:39:08 -0600},
	Doi = {10.1103/PhysRevLett.50.1153},
	Issue = {15},
	Journal = {Phys. Rev. Lett.},
	Month = {Apr},
	Numpages = {0},
	Pages = {1153--1156},
	Publisher = {American Physical Society},
	Title = {Nonlinear Field Theory of Large-Spin Heisenberg Antiferromagnets: Semiclassically Quantized Solitons of the One-Dimensional Easy-Axis N\'eel State},
	Url = {https://link.aps.org/doi/10.1103/PhysRevLett.50.1153},
	Volume = {50},
	Year = {1983},
	Bdsk-Url-1 = {https://link.aps.org/doi/10.1103/PhysRevLett.50.1153},
	Bdsk-Url-2 = {https://doi.org/10.1103/PhysRevLett.50.1153}}

@article{Venuti_2005,
	Author = {Venuti, L Campos and Boschi, C Degli Esposti and Ercolessi, E and Ortolani, F and Morandi, G and Pasini, S and Roncaglia, M},
	Date-Added = {2019-11-10 08:27:49 -0600},
	Date-Modified = {2019-11-10 08:30:09 -0600},
	Doi = {10.1088/1742-5468/2005/02/l02004},
	Issn = {1742-5468},
	Journal = {Journal of Statistical Mechanics: Theory and Experiment},
	Month = {Feb},
	Number = {02},
	Pages = {L02004},
	Publisher = {IOP Publishing},
	Title = {Particle content of the nonlinear sigma model with a $\theta$-term: a lattice model investigation},
	Url = {http://dx.doi.org/10.1088/1742-5468/2005/02/L02004},
	Volume = {2005},
	Year = {2005},
	Bdsk-Url-1 = {http://dx.doi.org/10.1088/1742-5468/2005/02/L02004},
	Bdsk-Url-2 = {http://dx.doi.org/10.1088/1742-5468/2005/02/l02004}}

@article{Rao_1997,
	Abstract = {We study the antiferromagnetic spin chain with both dimerization and frustration. The classical ground state has three phases, a N{\~A}{\copyright}el phase, a spiral phase and a collinear phase, which we study through a nonlinear sigma-model approach. In the spiral phase, the field theory becomes  and Lorentz invariant at long distances, a model which is exactly solvable. The low-energy spectrum is doubly degenerate with massive `elementary' spin-1/2 particles and `two-particle' triplet and singlet physical excitations. The field theory also supports  solitons which lead to a double degeneracy of the ground state for half-integer spins (when there is no dimerization).},
	Author = {Sumathi Rao and Diptiman Sen},
	Date-Added = {2019-11-10 08:25:07 -0600},
	Date-Modified = {2019-11-10 08:25:07 -0600},
	Doi = {10.1088/0953-8984/9/8/012},
	Journal = {Journal of Physics: Condensed Matter},
	Month = {feb},
	Number = {8},
	Pages = {1831--1839},
	Publisher = {{IOP} Publishing},
	Title = {Field theories for frustrated antiferromagnetic spin chains},
	Url = {https://doi.org/10.1088%2F0953-8984%2F9%2F8%2F012},
	Volume = {9},
	Year = 1997,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0953-8984%2F9%2F8%2F012},
	Bdsk-Url-2 = {https://doi.org/10.1088/0953-8984/9/8/012}}

@article{Schliemann_1998,
	Abstract = {We use spin-coherent states as the basis of a time-dependent variational  ansatz for a semiclassical description of a large family of Heisenberg models. In addition to following common approaches we also evaluate the square variance  of the Hamiltonian in terms of coherent states. This quantity turns out to have a natural interpretation with respect to time-dependent solutions of the equations of motion and allows an estimate of quantum fluctuations in a semiclassical regime to be made. The general results are applied to solitons, instantons and vortices in several one- and two-dimensional models.},
	Author = {John Schliemann and Franz G Mertens},
	Date-Added = {2019-11-09 10:09:59 -0600},
	Date-Modified = {2019-11-09 10:09:59 -0600},
	Doi = {10.1088/0953-8984/10/5/016},
	Journal = {Journal of Physics: Condensed Matter},
	Month = {feb},
	Number = {5},
	Pages = {1091--1102},
	Publisher = {{IOP} Publishing},
	Title = {Semiclassical description of Heisenberg models via spin-coherent states},
	Url = {https://doi.org/10.1088%2F0953-8984%2F10%2F5%2F016},
	Volume = {10},
	Year = 1998,
	Bdsk-Url-1 = {https://doi.org/10.1088%2F0953-8984%2F10%2F5%2F016},
	Bdsk-Url-2 = {https://doi.org/10.1088/0953-8984/10/5/016}}

@article{1971JPhA....4..313R,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/1971JPhA....4..313R},
	Author = {{Radcliffe}, J.~M.},
	Date-Added = {2019-11-07 16:17:34 -0600},
	Date-Modified = {2019-11-07 16:17:34 -0600},
	Doi = {10.1088/0305-4470/4/3/009},
	Journal = {Journal of Physics A Mathematical General},
	Month = {May},
	Number = {3},
	Pages = {313-323},
	Title = {{Some properties of coherent spin states}},
	Volume = {4},
	Year = {1971},
	Bdsk-Url-1 = {https://doi.org/10.1088/0305-4470/4/3/009}}

@article{Castillejo:1989hq,
	Author = {Castillejo, L. and Jones, P. S. J. and Jackson, A. D. and Verbaarschot, J. J. M. and Jackson, A.},
	Date-Added = {2019-11-02 14:18:58 -0600},
	Date-Modified = {2019-11-02 14:18:58 -0600},
	Doi = {10.1016/0375-9474(89)90161-9},
	Journal = {Nucl. Phys.},
	Pages = {801-812},
	Reportnumber = {Print-89-0195 (UNIV.COLL.,LONDON)},
	Slaccitation = {%%CITATION = NUPHA,A501,801;%%},
	Title = {{DENSE SKYRMION SYSTEMS}},
	Volume = {A501},
	Year = {1989},
	Bdsk-Url-1 = {https://doi.org/10.1016/0375-9474(89)90161-9}}

@article{GOLDHABER1987231,
	Abstract = {The symmetry of the classical Skyrme crystal considered by Klebanov and by W{\~A}{\OE}st, Brown and Jackson can be enlarged, implying that the crystal is a body-centered cubic lattice of half-skyrmions instead of a primitive cubic lattice of skyrmions.},
	Author = {Alfred S. Goldhaber and N.S. Manton},
	Date-Added = {2019-11-02 14:07:50 -0600},
	Date-Modified = {2019-11-02 14:07:50 -0600},
	Doi = {https://doi.org/10.1016/0370-2693(87)91502-4},
	Issn = {0370-2693},
	Journal = {Physics Letters B},
	Number = {2},
	Pages = {231 - 234},
	Title = {Maximal symmetry of the Skyrme crystal},
	Url = {http://www.sciencedirect.com/science/article/pii/0370269387915024},
	Volume = {198},
	Year = {1987},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/0370269387915024},
	Bdsk-Url-2 = {https://doi.org/10.1016/0370-2693(87)91502-4}}

@article{Klebanov:1985qi,
	Author = {Klebanov, Igor R.},
	Date-Added = {2019-11-02 13:48:15 -0600},
	Date-Modified = {2019-11-02 13:48:15 -0600},
	Doi = {10.1016/0550-3213(85)90068-9},
	Journal = {Nucl. Phys.},
	Pages = {133-143},
	Reportnumber = {Print-85-0469 (PRINCETON)},
	Slaccitation = {%%CITATION = NUPHA,B262,133;%%},
	Title = {{Nuclear Matter in the Skyrme Model}},
	Volume = {B262},
	Year = {1985},
	Bdsk-Url-1 = {https://doi.org/10.1016/0550-3213(85)90068-9}}

@article{Kugler:1988mu,
	Author = {Kugler, M. and Shtrikman, S.},
	Date-Added = {2019-11-02 13:47:38 -0600},
	Date-Modified = {2019-11-02 13:47:38 -0600},
	Doi = {10.1016/0370-2693(88)90653-3},
	Journal = {Phys. Lett.},
	Pages = {491-494},
	Reportnumber = {WIS-88-16-PH},
	Slaccitation = {%%CITATION = PHLTA,B208,491;%%},
	Title = {{A NEW SKYRMION CRYSTAL}},
	Volume = {B208},
	Year = {1988},
	Bdsk-Url-1 = {https://doi.org/10.1016/0370-2693(88)90653-3}}

@article{Perapechka:2017yyc,
	Archiveprefix = {arXiv},
	Author = {Perapechka, Ilya and Shnir, Yakov},
	Date-Added = {2019-11-02 11:53:26 -0600},
	Date-Modified = {2019-11-02 11:53:26 -0600},
	Doi = {10.1103/PhysRevD.96.045013},
	Eprint = {1703.10673},
	Journal = {Phys. Rev.},
	Number = {4},
	Pages = {045013},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1703.10673;%%},
	Title = {{Crystal structures in generalized Skyrme model}},
	Volume = {D96},
	Year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.96.045013}}

@article{Piette_1995,
	Author = {Piette, B. M. A. G. and Schroers, B. J. and Zakrzewski, W. J.},
	Date-Added = {2019-10-31 12:46:19 -0600},
	Date-Modified = {2019-10-31 12:46:19 -0600},
	Doi = {10.1007/bf01571317},
	Issn = {1434-6052},
	Journal = {Zeitschrift f{\"u}r Physik C Particles and Fields},
	Month = {Mar},
	Number = {1},
	Pages = {165--174},
	Publisher = {Springer Science and Business Media LLC},
	Title = {Multisolitons in a two-dimensional Skyrme model},
	Url = {http://dx.doi.org/10.1007/BF01571317},
	Volume = {65},
	Year = {1995},
	Bdsk-Url-1 = {http://dx.doi.org/10.1007/BF01571317},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/bf01571317}}

@misc{schroers2019solvable,
	Archiveprefix = {arXiv},
	Author = {Bernd Schroers},
	Date-Added = {2019-10-30 19:26:37 -0600},
	Date-Modified = {2019-10-30 19:26:37 -0600},
	Eprint = {1910.13907},
	Primaryclass = {cond-mat.mes-hall},
	Title = {Solvable Models for Magnetic Skyrmions},
	Year = {2019}}

@article{Saadatmand_2015,
	Author = {Saadatmand, S. N. and Powell, B. J. and McCulloch, I. P.},
	Date-Added = {2019-10-29 19:11:22 -0600},
	Date-Modified = {2019-10-29 19:11:22 -0600},
	Doi = {10.1103/physrevb.91.245119},
	Issn = {1550-235X},
	Journal = {Physical Review B},
	Month = {Jun},
	Number = {24},
	Publisher = {American Physical Society (APS)},
	Title = {Phase diagram of thespin−12triangularJ1−J2Heisenberg model on a three-leg cylinder},
	Url = {http://dx.doi.org/10.1103/PhysRevB.91.245119},
	Volume = {91},
	Year = {2015},
	Bdsk-Url-1 = {http://dx.doi.org/10.1103/PhysRevB.91.245119},
	Bdsk-Url-2 = {http://dx.doi.org/10.1103/physrevb.91.245119}}

@article{1992PhRvB..45.7832C,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/1992PhRvB..45.7832C},
	Author = {{Ceccatto}, H.~A. and {Gazza}, C.~J. and {Trumper}, A.~E.},
	Date-Added = {2019-10-29 19:01:47 -0600},
	Date-Modified = {2019-10-29 19:13:47 -0600},
	Doi = {10.1103/PhysRevB.45.7832},
	Journal = {prb},
	Keywords = {Spin waves, Quantized spin models, Antiferromagnetics},
	Month = apr,
	Pages = {7832-7836},
	Title = {{J$_{1}$-J$_{2}$ model: Energy, correlations, and order-parameter fluctuations on finite lattices}},
	Volume = 45,
	Year = 1992,
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevB.45.7832}}

@article{1989PhRvL..63.2148D,
	Adsnote = {Provided by the SAO/NASA Astrophysics Data System},
	Adsurl = {https://ui.adsabs.harvard.edu/abs/1989PhRvL..63.2148D},
	Author = {{Dagotto}, E. and {Moreo}, A.},
	Date-Added = {2019-10-29 18:57:03 -0600},
	Date-Modified = {2019-10-29 18:57:03 -0600},
	Doi = {10.1103/PhysRevLett.63.2148},
	Journal = {Physical Review Letters},
	Keywords = {Antiferromagnetism, High Temperature Superconductors, Lattice Parameters, Phase Diagrams, Solid State Physics, Spin, Broken Symmetry, Ground State, Heisenberg Theory},
	Month = nov,
	Pages = {2148-2151},
	Title = {{Phase diagram of the frustrated spin-1/2 Heisenberg antiferromagnet in two dimensions}},
	Volume = 63,
	Year = 1989,
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevLett.63.2148}}

@article{Nawa:2008uv,
	Archiveprefix = {arXiv},
	Author = {Nawa, Kanabu and Suganuma, Hideo and Kojo, Toru},
	Date-Added = {2019-10-29 11:46:04 -0600},
	Date-Modified = {2019-10-29 11:46:04 -0600},
	Doi = {10.1103/PhysRevD.79.026005},
	Eprint = {0810.1005},
	Journal = {Phys. Rev.},
	Pages = {026005},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:0810.1005;%%},
	Title = {{Brane-induced Skyrmion on S**3: Baryonic matter in holographic QCD}},
	Volume = {D79},
	Year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.79.026005}}

@article{Nastase:2005pb,
	Archiveprefix = {arXiv},
	Author = {Nastase, Horatiu},
	Date-Added = {2019-10-29 11:17:07 -0600},
	Date-Modified = {2019-10-29 11:17:07 -0600},
	Eprint = {hep-th/0512171},
	Primaryclass = {hep-th},
	Reportnumber = {BROWN-HET-1458},
	Slaccitation = {%%CITATION = HEP-TH/0512171;%%},
	Title = {{DBI skyrmion, high energy (large s) scattering and fireball production}},
	Year = {2005}}

@article{Pavlovsky:2002bx,
	Archiveprefix = {arXiv},
	Author = {Pavlovsky, O. V.},
	Date-Added = {2019-10-29 11:16:47 -0600},
	Date-Modified = {2019-10-29 11:16:47 -0600},
	Doi = {10.1016/S0370-2693(02)01967-6},
	Eprint = {hep-ph/0204313},
	Journal = {Phys. Lett.},
	Pages = {202},
	Primaryclass = {hep-ph},
	Slaccitation = {%%CITATION = HEP-PH/0204313;%%},
	Title = {{Chiral Born-Infeld theory: Topological spherically symmetrical solitons}},
	Volume = {B538},
	Year = {2002},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0370-2693(02)01967-6}}

@article{Tong:2014yla,
	Archiveprefix = {arXiv},
	Author = {Tong, David and Wong, Kenny},
	Date-Added = {2019-10-28 10:14:43 -0600},
	Date-Modified = {2019-10-28 10:14:43 -0600},
	Doi = {10.1007/JHEP06(2014)048},
	Eprint = {1401.6167},
	Journal = {JHEP},
	Pages = {048},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1401.6167;%%},
	Title = {{Monopoles and Wilson Lines}},
	Volume = {06},
	Year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP06(2014)048}}

@article{Zahed:1986qz,
	Author = {Zahed, I. and Brown, G. E.},
	Date-Added = {2019-10-26 14:38:04 -0600},
	Date-Modified = {2019-10-26 14:38:04 -0600},
	Doi = {10.1016/0370-1573(86)90142-0},
	Journal = {Phys. Rept.},
	Pages = {1-102},
	Reportnumber = {PRINT-86-0160 (STONY-BROOK)},
	Slaccitation = {%%CITATION = PRPLC,142,1;%%},
	Title = {{The Skyrme Model}},
	Volume = {142},
	Year = {1986},
	Bdsk-Url-1 = {https://doi.org/10.1016/0370-1573(86)90142-0}}

@article{Arnowitt:1962hi,
	Archiveprefix = {arXiv},
	Author = {Arnowitt, Richard L. and Deser, Stanley and Misner, Charles W.},
	Date-Added = {2019-10-25 22:18:46 -0600},
	Date-Modified = {2019-10-25 22:18:46 -0600},
	Doi = {10.1007/s10714-008-0661-1},
	Eprint = {gr-qc/0405109},
	Journal = {Gen. Rel. Grav.},
	Pages = {1997-2027},
	Primaryclass = {gr-qc},
	Slaccitation = {%%CITATION = GR-QC/0405109;%%},
	Title = {{The Dynamics of general relativity}},
	Volume = {40},
	Year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1007/s10714-008-0661-1}}

@article{Sutcliffe:2010et,
	Archiveprefix = {arXiv},
	Author = {Sutcliffe, Paul},
	Date-Added = {2019-10-25 17:34:49 -0600},
	Date-Modified = {2019-10-25 17:34:49 -0600},
	Doi = {10.1007/JHEP08(2010)019},
	Eprint = {1003.0023},
	Journal = {JHEP},
	Pages = {019},
	Primaryclass = {hep-th},
	Reportnumber = {DCPT-10-09},
	Slaccitation = {%%CITATION = ARXIV:1003.0023;%%},
	Title = {{Skyrmions, instantons and holography}},
	Volume = {08},
	Year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP08(2010)019}}

@article{Son:2003et,
	Archiveprefix = {arXiv},
	Author = {Son, D. T. and Stephanov, M. A.},
	Date-Added = {2019-10-25 17:24:18 -0600},
	Date-Modified = {2019-10-25 17:24:18 -0600},
	Doi = {10.1103/PhysRevD.69.065020},
	Eprint = {hep-ph/0304182},
	Journal = {Phys. Rev.},
	Pages = {065020},
	Primaryclass = {hep-ph},
	Reportnumber = {INT-PUB-03-07},
	Slaccitation = {%%CITATION = HEP-PH/0304182;%%},
	Title = {{QCD and dimensional deconstruction}},
	Volume = {D69},
	Year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.69.065020}}

@article{Witten:1995im,
	Archiveprefix = {arXiv},
	Author = {Witten, Edward},
	Date-Added = {2019-10-25 15:03:22 -0600},
	Date-Modified = {2019-10-25 15:03:22 -0600},
	Doi = {10.1016/0550-3213(95)00610-9},
	Eprint = {hep-th/9510135},
	Journal = {Nucl. Phys.},
	Pages = {335-350},
	Primaryclass = {hep-th},
	Reportnumber = {IASSNS-HEP-95-83},
	Slaccitation = {%%CITATION = HEP-TH/9510135;%%},
	Title = {{Bound states of strings and p-branes}},
	Volume = {B460},
	Year = {1996},
	Bdsk-Url-1 = {https://doi.org/10.1016/0550-3213(95)00610-9}}

@article{Brecher:1998su,
	Archiveprefix = {arXiv},
	Author = {Brecher, D. and Perry, M. J.},
	Date-Added = {2019-10-25 15:00:04 -0600},
	Date-Modified = {2019-10-25 15:00:04 -0600},
	Doi = {10.1016/S0550-3213(98)00297-1},
	Eprint = {hep-th/9801127},
	Journal = {Nucl. Phys.},
	Pages = {121-141},
	Primaryclass = {hep-th},
	Reportnumber = {DAMTP-R-98-02},
	Slaccitation = {%%CITATION = HEP-TH/9801127;%%},
	Title = {{Bound states of D-branes and the nonAbelian Born-Infeld action}},
	Volume = {B527},
	Year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0550-3213(98)00297-1}}

@article{Atiyah:2004nh,
	Archiveprefix = {arXiv},
	Author = {Atiyah, Michael and Sutcliffe, Paul},
	Date-Added = {2019-10-25 14:54:00 -0600},
	Date-Modified = {2019-10-25 14:54:00 -0600},
	Doi = {10.1016/j.physletb.2004.11.015},
	Eprint = {hep-th/0411052},
	Journal = {Phys. Lett.},
	Pages = {106-114},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = HEP-TH/0411052;%%},
	Title = {{Skyrmions, instantons, mass and curvature}},
	Volume = {B605},
	Year = {2005},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.physletb.2004.11.015}}

@article{Tseytlin:1997csa,
	Archiveprefix = {arXiv},
	Author = {Tseytlin, Arkady A.},
	Date-Added = {2019-10-25 14:36:24 -0600},
	Date-Modified = {2019-10-25 14:36:24 -0600},
	Doi = {10.1016/S0550-3213(97)00354-4},
	Eprint = {hep-th/9701125},
	Journal = {Nucl. Phys.},
	Pages = {41-52},
	Primaryclass = {hep-th},
	Reportnumber = {CERN-TH-97-009, CERN-TH-97-09, CERN-TH-97-9, IMPERIAL-TP-96-97-17},
	Slaccitation = {%%CITATION = HEP-TH/9701125;%%},
	Title = {{On nonAbelian generalization of Born-Infeld action in string theory}},
	Volume = {B501},
	Year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0550-3213(97)00354-4}}

@article{Hashimoto:1997gm,
	Archiveprefix = {arXiv},
	Author = {Hashimoto, Akikazu and Taylor, Washington},
	Date-Added = {2019-10-25 14:35:47 -0600},
	Date-Modified = {2019-10-25 14:35:47 -0600},
	Doi = {10.1016/S0550-3213(97)00399-4},
	Eprint = {hep-th/9703217},
	Journal = {Nucl. Phys.},
	Pages = {193-219},
	Primaryclass = {hep-th},
	Reportnumber = {PUPT-1693},
	Slaccitation = {%%CITATION = HEP-TH/9703217;%%},
	Title = {{Fluctuation spectra of tilted and intersecting D-branes from the Born-Infeld action}},
	Volume = {B503},
	Year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0550-3213(97)00399-4}}

@article{Argyres:1989qr,
	Author = {Argyres, Philip C. and Nappi, Chiara R.},
	Date-Added = {2019-10-25 14:33:46 -0600},
	Date-Modified = {2019-10-25 14:33:46 -0600},
	Doi = {10.1016/0550-3213(90)90305-W},
	Journal = {Nucl. Phys.},
	Pages = {151-173},
	Reportnumber = {IASSNS-HEP-89/42},
	Slaccitation = {%%CITATION = NUPHA,B330,151;%%},
	Title = {{Spin 1 Effective Actions From Open Strings}},
	Volume = {B330},
	Year = {1990},
	Bdsk-Url-1 = {https://doi.org/10.1016/0550-3213(90)90305-W}}

@article{Atiyah:1989dq,
	Author = {Atiyah, M. F. and Manton, N. S.},
	Date-Added = {2019-10-25 14:19:03 -0600},
	Date-Modified = {2019-10-25 14:19:03 -0600},
	Doi = {10.1016/0370-2693(89)90340-7},
	Journal = {Phys. Lett.},
	Pages = {438-442},
	Reportnumber = {DAMTP-89-07},
	Slaccitation = {%%CITATION = PHLTA,B222,438;%%},
	Title = {{Skyrmions From Instantons}},
	Volume = {B222},
	Year = {1989},
	Bdsk-Url-1 = {https://doi.org/10.1016/0370-2693(89)90340-7}}

@book{Johnson:2003gi,
	Author = {Johnson, Clifford V.},
	Date-Added = {2019-10-25 12:06:09 -0600},
	Date-Modified = {2019-10-25 12:06:09 -0600},
	Doi = {10.1017/CBO9780511606540},
	Isbn = {9780511057694, 9780521030052, 9780521809122, 9780511606540},
	Publisher = {Cambridge University Press},
	Series = {Cambridge Monographs on Mathematical Physics},
	Slaccitation = {%%CITATION = INSPIRE-612496;%%},
	Title = {{D-branes}},
	Url = {http://books.cambridge.org/0521809126.htm},
	Year = {2005},
	Bdsk-Url-1 = {http://books.cambridge.org/0521809126.htm},
	Bdsk-Url-2 = {https://doi.org/10.1017/CBO9780511606540}}

@article{Polchinski:1995mt,
	Archiveprefix = {arXiv},
	Author = {Polchinski, Joseph},
	Date-Added = {2019-10-25 12:05:08 -0600},
	Date-Modified = {2019-10-25 12:05:08 -0600},
	Doi = {10.1103/PhysRevLett.75.4724},
	Eprint = {hep-th/9510017},
	Journal = {Phys. Rev. Lett.},
	Pages = {4724-4727},
	Primaryclass = {hep-th},
	Reportnumber = {NSF-ITP-95-122},
	Slaccitation = {%%CITATION = HEP-TH/9510017;%%},
	Title = {{Dirichlet Branes and Ramond-Ramond charges}},
	Volume = {75},
	Year = {1995},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevLett.75.4724}}

@inproceedings{Schwarz:2001ps,
	Archiveprefix = {arXiv},
	Author = {Schwarz, John H.},
	Booktitle = {{Strings 2001: International Conference Mumbai, India, January 5-10, 2001}},
	Date-Added = {2019-10-25 12:03:25 -0600},
	Date-Modified = {2019-10-25 12:03:25 -0600},
	Eprint = {hep-th/0103165},
	Primaryclass = {hep-th},
	Reportnumber = {CALT-68-2322, CITUSC-01-006},
	Slaccitation = {%%CITATION = HEP-TH/0103165;%%},
	Title = {{Comments on Born-Infeld theory}},
	Year = {2001}}

@article{Brown:2009eh,
	Archiveprefix = {arXiv},
	Author = {Brown, Gerald E. and Rho, Mannque},
	Date-Added = {2019-10-12 07:21:54 -0600},
	Date-Modified = {2019-10-12 07:21:54 -0600},
	Eprint = {0907.1963},
	Primaryclass = {nucl-th},
	Slaccitation = {%%CITATION = ARXIV:0907.1963;%%},
	Title = {{The Multifaceted Skyrmion}},
	Year = {2009}}

@article{Elliot-Ripley:2015hoa,
	Archiveprefix = {arXiv},
	Author = {Elliot-Ripley, Matthew and Winyard, Thomas},
	Date-Added = {2019-10-12 06:58:03 -0600},
	Date-Modified = {2019-10-12 06:58:03 -0600},
	Doi = {10.1007/JHEP09(2015)009},
	Eprint = {1507.05928},
	Journal = {JHEP},
	Pages = {009},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1507.05928;%%},
	Title = {{Baby Skyrmions in AdS}},
	Volume = {09},
	Year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP09(2015)009}}

@article{Sakai:2005yt,
	Archiveprefix = {arXiv},
	Author = {Sakai, Tadakatsu and Sugimoto, Shigeki},
	Date-Added = {2019-10-12 06:43:41 -0600},
	Date-Modified = {2019-10-12 06:43:41 -0600},
	Doi = {10.1143/PTP.114.1083},
	Eprint = {hep-th/0507073},
	Journal = {Prog. Theor. Phys.},
	Pages = {1083-1118},
	Primaryclass = {hep-th},
	Reportnumber = {YITP-05-36, IU-MSTP-71},
	Slaccitation = {%%CITATION = HEP-TH/0507073;%%},
	Title = {{More on a holographic dual of QCD}},
	Volume = {114},
	Year = {2005},
	Bdsk-Url-1 = {https://doi.org/10.1143/PTP.114.1083}}

@article{Sakai:2004cn,
	Archiveprefix = {arXiv},
	Author = {Sakai, Tadakatsu and Sugimoto, Shigeki},
	Date-Added = {2019-10-12 06:38:52 -0600},
	Date-Modified = {2019-10-12 06:38:52 -0600},
	Doi = {10.1143/PTP.113.843},
	Eprint = {hep-th/0412141},
	Journal = {Prog. Theor. Phys.},
	Pages = {843-882},
	Primaryclass = {hep-th},
	Reportnumber = {IU-MSTP-63, YITP-04-70},
	Slaccitation = {%%CITATION = HEP-TH/0412141;%%},
	Title = {{Low energy hadron physics in holographic QCD}},
	Volume = {113},
	Year = {2005},
	Bdsk-Url-1 = {https://doi.org/10.1143/PTP.113.843}}

@article{Ma:2016npf,
	Archiveprefix = {arXiv},
	Author = {Ma, Yong-Liang and Harada, Masayasu},
	Date-Added = {2019-10-12 06:31:50 -0600},
	Date-Modified = {2019-10-12 06:31:50 -0600},
	Eprint = {1604.04850},
	Primaryclass = {hep-ph},
	Slaccitation = {%%CITATION = ARXIV:1604.04850;%%},
	Title = {{Lecture notes on the Skyrme model}},
	Year = {2016}}

@incollection{Hartnoll:2011fn,
	Archiveprefix = {arXiv},
	Author = {Hartnoll, Sean A.},
	Booktitle = {Black holes in higher dimensions},
	Date-Added = {2019-10-08 09:31:55 -0600},
	Date-Modified = {2019-10-08 09:31:55 -0600},
	Editor = {Horowitz, Gary T.},
	Eprint = {1106.4324},
	Pages = {387-419},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1106.4324;%%},
	Title = {{Horizons, holography and condensed matter}},
	Year = {2012}}

@article{Salvio:2012at,
	Archiveprefix = {arXiv},
	Author = {Salvio, Alberto},
	Date-Added = {2019-10-08 09:30:48 -0600},
	Date-Modified = {2019-10-08 09:30:48 -0600},
	Doi = {10.1007/JHEP09(2012)134},
	Eprint = {1207.3800},
	Journal = {JHEP},
	Pages = {134},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1207.3800;%%},
	Title = {{Holographic Superfluids and Superconductors in Dilaton-Gravity}},
	Volume = {09},
	Year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP09(2012)134}}

@article{Herdeiro:2016xnp,
	Archiveprefix = {arXiv},
	Author = {Herdeiro, Carlos and Radu, Eugen},
	Date-Added = {2019-10-07 09:56:24 -0600},
	Date-Modified = {2019-10-07 09:56:24 -0600},
	Doi = {10.1016/j.physletb.2016.04.004},
	Eprint = {1602.06990},
	Journal = {Phys. Lett.},
	Pages = {268-274},
	Primaryclass = {gr-qc},
	Slaccitation = {%%CITATION = ARXIV:1602.06990;%%},
	Title = {{Einstein--Maxwell--Anti-de-Sitter spinning solitons}},
	Volume = {B757},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.physletb.2016.04.004}}

@article{Yurova:2001mp,
	Archiveprefix = {arXiv},
	Author = {Yurova, Maria V.},
	Date-Added = {2019-10-07 09:55:11 -0600},
	Date-Modified = {2019-10-07 09:55:11 -0600},
	Doi = {10.1023/A:1001955710550},
	Eprint = {gr-qc/0101037},
	Journal = {Gen. Rel. Grav.},
	Pages = {2219-2227},
	Primaryclass = {gr-qc},
	Slaccitation = {%%CITATION = GR-QC/0101037;%%},
	Title = {{Soliton solution in dilaton Maxwell gravity}},
	Volume = {32},
	Year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1023/A:1001955710550}}

@article{Blazquez-Salcedo:2016vwa,
	Archiveprefix = {arXiv},
	Author = {Bl{\'a}zquez-Salcedo, Jose Luis and Kunz, Jutta and Navarro-L{\'e}rida, Francisco and Radu, Eugen},
	Date-Added = {2019-10-07 09:54:29 -0600},
	Date-Modified = {2019-10-07 09:54:29 -0600},
	Doi = {10.3390/e18120438},
	Eprint = {1612.03747},
	Journal = {Entropy},
	Pages = {438},
	Primaryclass = {gr-qc},
	Slaccitation = {%%CITATION = ARXIV:1612.03747;%%},
	Title = {{Static Einstein-Maxwell Magnetic Solitons and Black Holes in an Odd Dimensional AdS Spacetime}},
	Volume = {18},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.3390/e18120438}}

@article{Dias:2011tj,
	Archiveprefix = {arXiv},
	Author = {Dias, Oscar J. C. and Figueras, Pau and Minwalla, Shiraz and Mitra, Prahar and Monteiro, Ricardo and Santos, Jorge E.},
	Date-Added = {2019-10-07 09:53:37 -0600},
	Date-Modified = {2019-10-07 09:53:37 -0600},
	Doi = {10.1007/JHEP08(2012)117},
	Eprint = {1112.4447},
	Journal = {JHEP},
	Pages = {117},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1112.4447;%%},
	Title = {{Hairy black holes and solitons in global $AdS_5$}},
	Volume = {08},
	Year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP08(2012)117}}

@article{Costa:2015gol,
	Archiveprefix = {arXiv},
	Author = {Costa, Miguel S. and Greenspan, Lauren and Oliveira, Miguel and Penedones, Jo{\~a}o and Santos, Jorge E.},
	Date-Added = {2019-10-07 09:48:37 -0600},
	Date-Modified = {2019-10-07 09:48:37 -0600},
	Doi = {10.1088/0264-9381/33/11/115011},
	Eprint = {1511.08505},
	Journal = {Class. Quant. Grav.},
	Number = {11},
	Pages = {115011},
	Primaryclass = {hep-th},
	Reportnumber = {CERN-TH-2016-078},
	Slaccitation = {%%CITATION = ARXIV:1511.08505;%%},
	Title = {{Polarised Black Holes in AdS}},
	Volume = {33},
	Year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1088/0264-9381/33/11/115011}}

@article{Gubser:2009qt,
	Archiveprefix = {arXiv},
	Author = {Gubser, Steven S. and Rocha, Fabio D.},
	Date-Added = {2019-10-07 08:39:32 -0600},
	Date-Modified = {2019-10-07 08:39:50 -0600},
	Doi = {10.1103/PhysRevD.81.046001},
	Eprint = {0911.2898},
	Journal = {Phys. Rev.},
	Pages = {046001},
	Primaryclass = {hep-th},
	Reportnumber = {PUPT-2321},
	Slaccitation = {%%CITATION = ARXIV:0911.2898;%%},
	Title = {{Peculiar properties of a charged dilatonic black hole in $AdS_5$}},
	Volume = {D81},
	Year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1103/PhysRevD.81.046001}}

@article{Ling:2013nxa,
	Archiveprefix = {arXiv},
	Author = {Ling, Yi and Niu, Chao and Wu, Jian-Pin and Xian, Zhuo-Yu},
	Date-Added = {2019-10-07 08:28:13 -0600},
	Date-Modified = {2019-10-07 08:28:13 -0600},
	Doi = {10.1007/JHEP11(2013)006},
	Eprint = {1309.4580},
	Journal = {JHEP},
	Pages = {006},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1309.4580;%%},
	Title = {{Holographic Lattice in Einstein-Maxwell-Dilaton Gravity}},
	Volume = {11},
	Year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP11(2013)006}}

@article{Horowitz:2012ky,
	Archiveprefix = {arXiv},
	Author = {Horowitz, Gary T. and Santos, Jorge E. and Tong, David},
	Date-Added = {2019-10-07 08:26:36 -0600},
	Date-Modified = {2019-10-07 08:26:36 -0600},
	Doi = {10.1007/JHEP07(2012)168},
	Eprint = {1204.0519},
	Journal = {JHEP},
	Pages = {168},
	Primaryclass = {hep-th},
	Slaccitation = {%%CITATION = ARXIV:1204.0519;%%},
	Title = {{Optical Conductivity with Holographic Lattices}},
	Volume = {07},
	Year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1007/JHEP07(2012)168}}

